VILA-U: a Unified Foundation Model Integrating Visual Understanding and Generation

VILA-U is a Unified foundation model that integrates Video, Image, Language understanding and generation. Traditional visual language models (VLMs) use separate modules for understanding and generating visual content, which can lead to misalignment and increased complexity. In contrast, VILA-U employs a single autoregressive next-token prediction framework for both tasks, eliminating the need for additional components like diffusion models. This approach not only simplifies the model but also achieves near state-of-the-art performance in visual language understanding and generation. The success of VILA-U is attributed to two main factors: the unified vision tower that aligns discrete visual tokens with textual inputs during pretraining, which enhances visual perception, and autoregressive image generation can achieve similar quality as diffusion models with high-quality dataset. This allows VILA-U to perform comparably to more complex models using a fully token-based autoregressive framework.

==> table/ablation_pretrain.tex <==
\begin{table}[h]
\setlength{\tabcolsep}{5.5pt}
\centering
\caption{Ablation study on the vision tower.}
\scalebox{0.65}{
\begin{tabular}{l l l | c | c c c c c c c c}
\toprule
Vision Encoder & Data size & Loss Type & Top-1 & {\bf VQAv2} & {\bf GQA} & {\bf VizWiz} & {\bf TextVQA} &  {\bf POPE} & {\bf MME} & {\bf SEED} & {\bf MM-Vet}\\
\midrule
ConvNext-Large & 25M & Reconstruction Only & / & 57.7 & 48.7 & 44.5 & 44.1 & 75.1 & 937.7 & 38.7 & 15.3 \\
ConvNext-Large & 25M & Contrastive + Reconstruction &  54.9 & 68.0 & 55.4 & 41.8 & 47.9 & 83.7 & 1219 & 50.4 & 20.8\\
\midrule
\rowcolor{mygray}ConvNext-Large & 700M & Contrastive + Reconstruction & 65.0 & 75.3 & 59.6 & 53.7 & 51.6 & 84.3 & 1324 & 56.3 & 25.1\\
\bottomrule
\end{tabular}
}
\label{tab:ablation_pretrain}
\end{table}

==> table/data_details.tex <==
\begin{table}[h]
\setlength{\tabcolsep}{5.5pt}
\centering
\caption{Datasets used in each phase and some details.}
\scalebox{0.8}{
\begin{tabular}{l|l}
\toprule
Phase & Datasets \\
\midrule
Vision Tower Training & COYO-700m \\
\midrule
Vision Tower Evaluation & ImageNet Validation set (50K image-label pairs)\\
\midrule
\multirow{2}{*}{Multi-modal Understanding Pre-training} & ShareGPT4V (1M [image, text] pairs) \\
& MMC4 (6M interleaved text and image data) \\
\midrule
\multirow{3}{*}{Multi-modal Generation Pre-training} & Internal database (15M high-quality [text, image] pairs)\\
& Panda (selected 200K) \\
& InterVid (selected 500k)\\
\midrule
Image-text Understanding Evaluation & VQAv2, GQA, VizWiz, TextVQA, POPE, MME, SEED, MM-Vet \\
\midrule
Video-text Understanding Evaluation & Activity Net, MSVD, MSRVTT, TGIF \\
\midrule
Visual Generation Evaluation & GenAI-Bench (527 text prompts) \\
\bottomrule
\end{tabular}
}
\label{tab:data_details}
\end{table}

==> table/hyperparameters.tex <==
\begin{table}[h]
  \centering
  \small
  \caption{Summary of hyperparameters configuration of \abbns.}
  \label{tab:training cfg}
  \setlength{\tabcolsep}{0.15cm}
  \renewcommand{\arraystretch}{1.4}
  % \begin{tabular}{l l m{6cm}}
  % \toprule
  % Stage & Configuration & Pretraining \\
  % \midrule
  % \multicolumn{3}{*}{Vision Tower Training} & & \\
  

  % \bottomrule
  % \end{tabular}
\begin{tblr}{
  colspec={|c|c|c|},
  hline{1,2,10,17},
  cell{2}{1} = {r=8}{m}, % multirow
  cell{10}{1} = {r=7}{m},
}
Training Stage & Configuration & Hyperparameter \\
Vision Tower Training & Vision Encoder pre-trained weights & CLIP-ConvNext-Large \\
 & Text Encoder pre-trained weights & CLIP-ConvNext-Large \\
 & Resolution & $256\times 256$ \\
 & Codebook vocabulary size & 16384 \\
 & Code shape & $16\times 16\times 4$ \\
 & Learning rate & $4.0\times 10^{-5}$ \\
 & Lr scheduler & cosine annealing\\
 & Global batch size & 4096 \\
 Multi-modal Pre-training & Language Model pre-trained weights & LLaMA-2-7B\\
 & Depth transformer size & 520M \\
 & Depth transformer layers & 6 \\
 & Depth transformer hidden size & 2560 \\
 & Learning rate & $5.0\times 10^{-5}$\\
 & Lr scheduler & cosine annealing \\
 & Global batch size & 512\\
\end{tblr}

\end{table}
